TALLRec: An Effective and Efficient Tuning Framework to Align Large Language Model with Recommendation

Large Language Models (LLMs) have demonstrated remarkable performance across diverse domains, thereby prompting researchers to explore their potential for use in recommendation systems. Initial attempts have leveraged the exceptional capabilities of LLMs, such as rich knowledge and strong generalization through In-context Learning, which involves phrasing the recommendation task as prompts. Nevertheless, the performance of LLMs in recommendation tasks remains suboptimal due to a substantial disparity between the training tasks for LLMs and recommendation tasks, as well as inadequate recommendation data during pre-training. To bridge the gap, we consider building a Large Recommendation Language Model by tunning LLMs with recommendation data. To this end, we propose an efficient and effective Tuning framework for Aligning LLMs with Recommendation, namely TALLRec. We have demonstrated that the proposed TALLRec framework can significantly enhance the recommendation capabilities of LLMs in the movie and book domains, even with a limited dataset of fewer than 100 samples. Additionally, the proposed framework is highly efficient and can be executed on a single RTX 3090 with LLaMA-7B. Furthermore, the fine-tuned LLM exhibits robust cross-domain generalization. Our code and data are available at https://github.com/SAI990323/TALLRec.

==> 00_ref_backup.tex <==

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

%Entries

@article{wei2021finetuned,
  title={Finetuned language models are zero-shot learners},
  author={Wei, Jason and Bosma, Maarten and Zhao, Vincent Y and Guu, Kelvin and Yu, Adams Wei and Lester, Brian and Du, Nan and Dai, Andrew M and Le, Quoc V},
  journal={arXiv preprint arXiv:2109.01652},
  year={2021}
}
@article{ouyang2022training,
  title={Training language models to follow instructions with human feedback},
  author={Ouyang, Long and Wu, Jeffrey and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll and Mishkin, Pamela and Zhang, Chong and Agarwal, Sandhini and Slama, Katarina and Ray, Alex and others},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={27730--27744},
  year={2022}
}
@article{sanh2021multitask,
  title={Multitask prompted training enables zero-shot task generalization},
  author={Sanh, Victor and Webson, Albert and Raffel, Colin and Bach, Stephen H and Sutawika, Lintang and Alyafeai, Zaid and Chaffin, Antoine and Stiegler, Arnaud and Scao, Teven Le and Raja, Arun and others},
  journal={arXiv preprint arXiv:2110.08207},
  year={2021}
}

@inproceedings{book_crossing,
author = {Ziegler, Cai-Nicolas and McNee, Sean M. and Konstan, Joseph A. and Lausen, Georg},
title = {Improving Recommendation Lists through Topic Diversification},
year = {2005},
isbn = {1595930469},
publisher = {Association for Computing Machinery},


booktitle = {Proceedings of the 14th International Conference on World Wide Web},
pages = {22–32},
numpages = {11},
series = {WWW '05}
}


@inproceedings{GRU4Rec,
  author    = {Bal{\'{a}}zs Hidasi and
               Alexandros Karatzoglou and
               Linas Baltrunas and
               Domonkos Tikk},
  title     = {Session-based Recommendations with Recurrent Neural Networks},
  booktitle = {ICLR},
  year      = {2016}
}

@inproceedings{Caser,
  title={Personalized top-n sequential recommendation via convolutional sequence embedding},
  author={Tang, Jiaxi and Wang, Ke},
  booktitle={WSDM},
  pages={565--573},
  year={2018}
}

@inproceedings{SASRec,
  title={Self-attentive sequential recommendation},
  author={Kang, Wang-Cheng and McAuley, Julian},
  booktitle={ICDM},
  pages={197--206},
  year={2018}
}

@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    publisher = "Association for Computational Linguistics",
    pages = "4171--4186",
}

@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}

@article{DROS,
  title={A Generic Learning Framework for Sequential Recommendation with Distribution Shifts},
  author={Yang, Zhengyi and He, Xiangnan and Zhang, Jizhi and Wu, Jiancan and Xin, Xin and Chen, Jiawei and Wang, Xiang},
  journal={Proceedings of the 46th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  year={2023}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

 @misc{sklearn,  
 title={Scikit-learn: Machine Learning in Python}, 
 journal={Journal of Machine Learning Research}, 
 author={Pedregosa, Fabian and Varoquaux, Gaël and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and Vanderplas, Jake and Passos, Alexandre and Cournapeau, David and Brucher, Matthieu and Perrot, Matthieu and Duchesnay, Edouard}, 
 year={2011}, 
 month={Feb} 
 }

 @inproceedings{seq_markov_1,
  title={Factorizing personalized markov chains for next-basket recommendation},
  author={Rendle, Steffen and Freudenthaler, Christoph and Schmidt-Thieme, Lars},
  booktitle={Proceedings of the 19th international conference on World wide web},
  pages={811--820},
  year={2010}
}

@inproceedings{seq_markov_2,
  title={Fusing similarity models with markov chains for sparse sequential recommendation},
  author={He, Ruining and McAuley, Julian},
  booktitle={2016 IEEE 16th international conference on data mining (ICDM)},
  pages={191--200},
  year={2016},
  organization={IEEE}
}

@inproceedings{seq_markov_3,
  title={Learning hierarchical representation model for nextbasket recommendation},
  author={Wang, Pengfei and Guo, Jiafeng and Lan, Yanyan and Xu, Jun and Wan, Shengxian and Cheng, Xueqi},
  booktitle={Proceedings of the 38th International ACM SIGIR conference on Research and Development in Information Retrieval},
  pages={403--412},
  year={2015}
}

@inproceedings{seq_markov_4,
  title={Learning and adaptivity in interactive recommender systems},
  author={Mahmood, Tariq and Ricci, Francesco},
  booktitle={Proceedings of the ninth international conference on Electronic commerce},
  pages={75--84},
  year={2007}
}

@article{seq_rec_1,
  author       = {Qiang Cui and
                  Shu Wu and
                  Qiang Liu and
                  Wen Zhong and
                  Liang Wang},
  title        = {{MV-RNN:} {A} Multi-View Recurrent Neural Network for Sequential Recommendation},
  journal      = {{IEEE} Trans. Knowl. Data Eng.},
  volume       = {32},
  number       = {2},
  pages        = {317--331},
  year         = {2020},



}

@inproceedings{seq_rec_2,
  title={Sequential user-based recurrent neural network recommendations},
  author={Donkers, Tim and Loepp, Benedikt and Ziegler, J{\"u}rgen},
  booktitle={Proceedings of the eleventh ACM conference on recommender systems},
  pages={152--160},
  year={2017}
}

@inproceedings{CNN_seq_1,
  author       = {Fajie Yuan and
                  Alexandros Karatzoglou and
                  Ioannis Arapakis and
                  Joemon M. Jose and
                  Xiangnan He},
  title        = {A Simple Convolutional Generative Network for Next Item Recommendation},
  booktitle    = {Proceedings of the Twelfth {ACM} International Conference on Web Search
                  and Data Mining, {WSDM} 2019, Melbourne, VIC, Australia, February
                  11-15, 2019},
  pages        = {582--590},
  publisher    = {{ACM}},
  year         = {2019},



}

@inproceedings{CNN_seq_2,
  author       = {An Yan and
                  Shuo Cheng and
                  Wang{-}Cheng Kang and
                  Mengting Wan and
                  Julian J. McAuley},

  title        = {CosRec: 2D Convolutional Neural Networks for Sequential Recommendation},
  booktitle    = {Proceedings of the 28th {ACM} International Conference on Information
                  and Knowledge Management, {CIKM} 2019, Beijing, China, November 3-7,
                  2019},
  pages        = {2173--2176},
  publisher    = {{ACM}},
  year         = {2019},



}

@inproceedings{attention_seq_1,
  author       = {Tingting Zhang and
                  Pengpeng Zhao and
                  Yanchi Liu and
                  Victor S. Sheng and
                  Jiajie Xu and
                  Deqing Wang and
                  Guanfeng Liu and
                  Xiaofang Zhou},
  title        = {Feature-level Deeper Self-Attention Network for Sequential Recommendation},
  booktitle    = {Proceedings of the Twenty-Eighth International Joint Conference on
                  Artificial Intelligence, {IJCAI} 2019, Macao, China, August 10-16,
                  2019},
  pages        = {4320--4326},
  publisher    = {ijcai.org},
  year         = {2019},



}

@article{attention_seq_2,
  author       = {Chengfeng Xu and
                  Jian Feng and
                  Pengpeng Zhao and
                  Fuzhen Zhuang and
                  Deqing Wang and
                  Yanchi Liu and
                  Victor S. Sheng},
  title        = {Long- and short-term self-attention network for sequential recommendation},
  journal      = {Neurocomputing},
  volume       = {423},
  pages        = {580--589},
  year         = {2021},



}

@article{seq_survey_1,
  author       = {Hui Fang and
                  Danning Zhang and
                  Yiheng Shu and
                  Guibing Guo},
  title        = {Deep Learning for Sequential Recommendation: Algorithms, Influential
                  Factors, and Evaluations},
  journal      = {{ACM} Trans. Inf. Syst.},
  volume       = {39},
  number       = {1},
  pages        = {10:1--10:42},
  year         = {2020},



}

@inproceedings{seq_survey_2,
  author       = {Shoujin Wang and
                  Liang Hu and
                  Yan Wang and
                  Longbing Cao and
                  Quan Z. Sheng and
                  Mehmet A. Orgun},
  title        = {Sequential Recommender Systems: Challenges, Progress and Prospects},
  booktitle    = {Proceedings of the Twenty-Eighth International Joint Conference on
                  Artificial Intelligence, {IJCAI} 2019, Macao, China, August 10-16,
                  2019},
  pages        = {6332--6338},
  publisher    = {ijcai.org},
  year         = {2019},



}

@inproceedings{pretrain_1,
  author       = {Yabo Ni and
                  Dan Ou and
                  Shichen Liu and
                  Xiang Li and
                  Wenwu Ou and
                  Anxiang Zeng and
                  Luo Si},
  title        = {Perceive Your Users in Depth: Learning Universal User Representations
                  from Multiple E-commerce Tasks},
  booktitle    = {Proceedings of the 24th {ACM} {SIGKDD} International Conference on
                  Knowledge Discovery {\&} Data Mining, {KDD} 2018, London, UK,
                  August 19-23, 2018},
  pages        = {596--605},
  publisher    = {{ACM}},
  year         = {2018},



}

@inproceedings{pretrain_2,
  author       = {Fajie Yuan and
                  Xiangnan He and
                  Alexandros Karatzoglou and
                  Liguang Zhang},
  title        = {Parameter-Efficient Transfer from Sequential Behaviors for User Modeling
                  and Recommendation},
  booktitle    = {Proceedings of the 43rd International {ACM} {SIGIR} conference on
                  research and development in Information Retrieval, {SIGIR} 2020, Virtual
                  Event, China, July 25-30, 2020},
  pages        = {1469--1478},
  publisher    = {{ACM}},
  year         = {2020},



}

@inproceedings{contrast_1,
  author       = {Ruihong Qiu and
                  Zi Huang and
                  Hongzhi Yin and
                  Zijian Wang},
  title        = {Contrastive Learning for Representation Degeneration Problem in Sequential
                  Recommendation},
  booktitle    = {{WSDM} '22: The Fifteenth {ACM} International Conference on Web Search
                  and Data Mining, Virtual Event / Tempe, AZ, USA, February 21 - 25,
                  2022},
  pages        = {813--823},
  publisher    = {{ACM}},
  year         = {2022},



}

@article{contrast_2,
  author       = {Ruihong Qiu and
                  Zi Huang and
                  Hongzhi Yin and
                  Zijian Wang},
  title        = {Contrastive Learning for Representation Degeneration Problem in Sequential
                  Recommendation},
  journal      = {CoRR},
  volume       = {abs/2110.05730},
  year         = {2021},

  eprinttype    = {arXiv},
  eprint       = {2110.05730},


}

@article{contrast_3,
  author       = {Ziyang Wang and
                  Huoyu Liu and
                  Wei Wei and
                  Yue Hu and
                  Xian{-}Ling Mao and
                  Shaojian He and
                  Rui Fang and
                  Dangyang Chen},
  title        = {Multi-level Contrastive Learning Framework for Sequential Recommendation},
  journal      = {CoRR},
  volume       = {abs/2208.13007},
  year         = {2022},

  eprinttype    = {arXiv},
  eprint       = {2208.13007},


}

@inproceedings{contrast_4,
  author       = {Xu Xie and
                  Fei Sun and
                  Zhaoyang Liu and
                  Shiwen Wu and
                  Jinyang Gao and
                  Jiandong Zhang and
                  Bolin Ding and
                  Bin Cui},
  title        = {Contrastive Learning for Sequential Recommendation},
  booktitle    = {38th {IEEE} International Conference on Data Engineering, {ICDE} 2022,
                  Kuala Lumpur, Malaysia, May 9-12, 2022},
  pages        = {1259--1273},
  publisher    = {{IEEE}},
  year         = {2022},



}

@inproceedings{debias_1,
  author       = {Sihao Ding and
                  Fuli Feng and
                  Xiangnan He and
                  Jinqiu Jin and
                  Wenjie Wang and
                  Yong Liao and
                  Yongdong Zhang},
  title        = {Interpolative Distillation for Unifying Biased and Debiased Recommendation},
  booktitle    = {{SIGIR} '22: The 45th International {ACM} {SIGIR} Conference on Research
                  and Development in Information Retrieval, Madrid, Spain, July 11 -
                  15, 2022},
  pages        = {40--49},
  publisher    = {{ACM}},
  year         = {2022},



}

@inproceedings{debias_2,
  author       = {Zhenlei Wang and
                  Shiqi Shen and
                  Zhipeng Wang and
                  Bo Chen and
                  Xu Chen and
                  Ji{-}Rong Wen},
  title        = {Unbiased Sequential Recommendation with Latent Confounders},
  booktitle    = {{WWW} '22: The {ACM} Web Conference 2022, Virtual Event, Lyon, France,
                  April 25 - 29, 2022},
  pages        = {2195--2204},
  publisher    = {{ACM}},
  year         = {2022},



}

@inproceedings{debias_3,
  author       = {Yu Zheng and
                  Chen Gao and
                  Xiang Li and
                  Xiangnan He and
                  Yong Li and
                  Depeng Jin},
  title        = {Disentangling User Interest and Conformity for Recommendation with
                  Causal Embedding},
  booktitle    = {{WWW} '21: The Web Conference 2021, Virtual Event / Ljubljana, Slovenia,
                  April 19-23, 2021},
  pages        = {2980--2991},
  publisher    = {{ACM} / {IW3C2}},
  year         = {2021},



}

@inproceedings{debias_4,
  author       = {Yang Zhang and
                  Fuli Feng and
                  Xiangnan He and
                  Tianxin Wei and
                  Chonggang Song and
                  Guohui Ling and
                  Yongdong Zhang},
  title        = {Causal Intervention for Leveraging Popularity Bias in Recommendation},
  booktitle    = {{SIGIR} '21: The 44th International {ACM} {SIGIR} Conference on Research
                  and Development in Information Retrieval, Virtual Event, Canada, July
                  11-15, 2021},
  pages        = {11--20},
  publisher    = {{ACM}},
  year         = {2021},



}

@inproceedings{group_dro_1,
  author       = {Hongyi Wen and
                  Xinyang Yi and
                  Tiansheng Yao and
                  Jiaxi Tang and
                  Lichan Hong and
                  Ed H. Chi},
  title        = {Distributionally-robust Recommendations for Improving Worst-case User
                  Experience},
  booktitle    = {{WWW} '22: The {ACM} Web Conference 2022, Virtual Event, Lyon, France,
                  April 25 - 29, 2022},
  pages        = {3606--3610},
  publisher    = {{ACM}},
  year         = {2022},



}
@article{lin2021few,
  title={Few-shot learning with multilingual language models},
  author={Lin, Xi Victoria and Mihaylov, Todor and Artetxe, Mikel and Wang, Tianlu and Chen, Shuohui and Simig, Daniel and Ott, Myle and Goyal, Naman and Bhosale, Shruti and Du, Jingfei and others},
  journal={arXiv preprint arXiv:2112.10668},
  year={2021}
}
@article{liang2022holistic,
  title={Holistic evaluation of language models},
  author={Liang, Percy and Bommasani, Rishi and Lee, Tony and Tsipras, Dimitris and Soylu, Dilara and Yasunaga, Michihiro and Zhang, Yian and Narayanan, Deepak and Wu, Yuhuai and Kumar, Ananya and others},
  journal={arXiv preprint arXiv:2211.09110},
  year={2022}
}

@inproceedings{LLM_rob_1,
  author       = {Dhruv Shah and
                  Blazej Osinski and
                  Brian Ichter and
                  Sergey Levine},
  title        = {LM-Nav: Robotic Navigation with Large Pre-Trained Models of Language,
                  Vision, and Action},
  booktitle    = {Conference on Robot Learning, CoRL 2022, 14-18 December 2022, Auckland,
                  New Zealand},
  series       = {Proceedings of Machine Learning Research},
  volume       = {205},
  pages        = {492--504},
  publisher    = {{PMLR}},
  year         = {2022},


}

@article{LLM_rob_2,
  author       = {Ted Xiao and
                  Harris Chan and
                  Pierre Sermanet and
                  Ayzaan Wahid and
                  Anthony Brohan and
                  Karol Hausman and
                  Sergey Levine and
                  Jonathan Tompson},
  title        = {Robotic Skill Acquisition via Instruction Augmentation with Vision-Language
                  Models},
  journal      = {CoRR},
  volume       = {abs/2211.11736},
  year         = {2022},

  eprinttype    = {arXiv},
  eprint       = {2211.11736},


}

@article{LLM_rob_3,
  author       = {Danny Driess and
                  Fei Xia and
                  Mehdi S. M. Sajjadi and
                  Corey Lynch and
                  Aakanksha Chowdhery and
                  Brian Ichter and
                  Ayzaan Wahid and
                  Jonathan Tompson and
                  Quan Vuong and
                  Tianhe Yu and
                  Wenlong Huang and
                  Yevgen Chebotar and
                  Pierre Sermanet and
                  Daniel Duckworth and
                  Sergey Levine and
                  Vincent Vanhoucke and
                  Karol Hausman and
                  Marc Toussaint and
                  Klaus Greff and
                  Andy Zeng and
                  Igor Mordatch and
                  Pete Florence},
  title        = {PaLM-E: An Embodied Multimodal Language Model},
  journal      = {CoRR},
  volume       = {abs/2303.03378},
  year         = {2023},

  eprinttype    = {arXiv},
  eprint       = {2303.03378},


}

@article{schick2023toolformer,
  title={Toolformer: Language models can teach themselves to use tools},
  author={Schick, Timo and Dwivedi-Yu, Jane and Dess{\`\i}, Roberto and Raileanu, Roberta and Lomeli, Maria and Zettlemoyer, Luke and Cancedda, Nicola and Scialom, Thomas},
  journal={arXiv preprint arXiv:2302.04761},
  year={2023}
}
@article{gao2023chat,
  title={Chat-REC: Towards Interactive and Explainable LLMs-Augmented Recommender System},
  author={Gao, Yunfan and Sheng, Tao and Xiang, Youlin and Xiong, Yun and Wang, Haofen and Zhang, Jiawei},
  journal={arXiv preprint arXiv:2303.14524},
  year={2023}
}
@article{wang2023zero,
  title={Zero-Shot Next-Item Recommendation using Large Pretrained Language Models},
  author={Wang, Lei and Lim, Ee-Peng},
  journal={arXiv preprint arXiv:2304.03153},
  year={2023}
}
@inproceedings{he2020lightgcn,
  title={Lightgcn: Simplifying and powering graph convolution network for recommendation},
  author={He, Xiangnan and Deng, Kuan and Wang, Xiang and Li, Yan and Zhang, Yongdong and Wang, Meng},
  booktitle={Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval},
  pages={639--648},
  year={2020}
}

@article{koren2009matrix,
  title={Matrix factorization techniques for recommender systems},
  author={Koren, Yehuda and Bell, Robert and Volinsky, Chris},
  journal={Computer},
  volume={42},
  number={8},
  pages={30--37},
  year={2009},
  publisher={IEEE}
}

@article{LLM_IR_1,
  author       = {Vitor Jeronymo and
                  Luiz Henrique Bonifacio and
                  Hugo Abonizio and
                  Marzieh Fadaee and
                  Roberto de Alencar Lotufo and
                  Jakub Zavrel and
                  Rodrigo Frassetto Nogueira},
  title        = {InPars-v2: Large Language Models as Efficient Dataset Generators for
                  Information Retrieval},
  journal      = {CoRR},
  volume       = {abs/2301.01820},
  year         = {2023},

  eprinttype    = {arXiv},
  eprint       = {2301.01820},


}

@article{LLM_IR_2,
  author       = {Liang Wang and
                  Nan Yang and
                  Furu Wei},
  title        = {Query2doc: Query Expansion with Large Language Models},
  journal      = {CoRR},
  volume       = {abs/2303.07678},
  year         = {2023},

  eprinttype    = {arXiv},
  eprint       = {2303.07678},


}

@article{LLM_IR_3,
  author       = {Matthew Jin and
                  Syed Shahriar and
                  Michele Tufano and
                  Xin Shi and
                  Shuai Lu and
                  Neel Sundaresan and
                  Alexey Svyatkovskiy},
  title        = {InferFix: End-to-End Program Repair with LLMs},
  journal      = {CoRR},
  volume       = {abs/2303.07263},
  year         = {2023},

  eprinttype    = {arXiv},
  eprint       = {2303.07263},


}


@article{chowdhery2022palm,
  title={Palm: Scaling language modeling with pathways},
  author={Chowdhery, Aakanksha and Narang, Sharan and Devlin, Jacob and Bosma, Maarten and Mishra, Gaurav and Roberts, Adam and Barham, Paul and Chung, Hyung Won and Sutton, Charles and Gehrmann, Sebastian and others},
  journal={arXiv preprint arXiv:2204.02311},
  year={2022}
}
@article{wei2022emergent,
  title={Emergent abilities of large language models},
  author={Wei, Jason and Tay, Yi and Bommasani, Rishi and Raffel, Colin and Zoph, Barret and Borgeaud, Sebastian and Yogatama, Dani and Bosma, Maarten and Zhou, Denny and Metzler, Donald and others},
  journal={arXiv preprint arXiv:2206.07682},
  year={2022}
}

@article{instruct_gen_1,
  author       = {Baolin Peng and
                  Chunyuan Li and
                  Pengcheng He and
                  Michel Galley and
                  Jianfeng Gao},
  title        = {Instruction Tuning with {GPT-4}},
  journal      = {CoRR},
  volume       = {abs/2304.03277},
  year         = {2023},

  eprinttype    = {arXiv},
  eprint       = {2304.03277},


}

@article{instruct_gen_2,
  author       = {Joel Jang and
                  Seungone Kim and
                  Seonghyeon Ye and
                  Doyoung Kim and
                  Lajanugen Logeswaran and
                  Moontae Lee and
                  Kyungjae Lee and
                  Minjoon Seo},
  title        = {Exploring the Benefits of Training Expert Language Models over Instruction
                  Tuning},
  journal      = {CoRR},
  volume       = {abs/2302.03202},
  year         = {2023},

  eprinttype    = {arXiv},
  eprint       = {2302.03202},


}

@article{instruct_gen_3,
  title={OPT-IML: Scaling Language Model Instruction Meta Learning through the Lens of Generalization},
  author={Iyer, Srinivasan and Lin, Xi Victoria and Pasunuru, Ramakanth and Mihaylov, Todor and Simig, D{\'a}niel and Yu, Ping and Shuster, Kurt and Wang, Tianlu and Liu, Qing and Koura, Punit Singh and others},
  journal={arXiv preprint arXiv:2212.12017},
  year={2022}
}

@inproceedings{lora,
  author       = {Edward J. Hu and
                  Yelong Shen and
                  Phillip Wallis and
                  Zeyuan Allen{-}Zhu and
                  Yuanzhi Li and
                  Shean Wang and
                  Lu Wang and
                  Weizhu Chen},
  title        = {LoRA: Low-Rank Adaptation of Large Language Models},
  booktitle    = {The Tenth International Conference on Learning Representations, {ICLR}
                  2022, Virtual Event, April 25-29, 2022},
  publisher    = {OpenReview.net},
  year         = {2022},


}
@article{cui2022m6,
  title={M6-Rec: Generative Pretrained Language Models are Open-Ended Recommender Systems},
  author={Cui, Zeyu and Ma, Jianxin and Zhou, Chang and Zhou, Jingren and Yang, Hongxia},
  journal={arXiv preprint arXiv:2205.08084},
  year={2022}
}
@inproceedings{hou2022towards,
  title={Towards Universal Sequence Representation Learning for Recommender Systems},
  author={Hou, Yupeng and Mu, Shanlei and Zhao, Wayne Xin and Li, Yaliang and Ding, Bolin and Wen, Ji-Rong},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={585--593},
    year={2022}
}
@article{chinchilla,
  title={Training compute-optimal large language models},
  author={Hoffmann, Jordan and Borgeaud, Sebastian and Mensch, Arthur and Buchatskaya, Elena and Cai, Trevor and Rutherford, Eliza and Casas, Diego de Las and Hendricks, Lisa Anne and Welbl, Johannes and Clark, Aidan and others},
  journal={arXiv preprint arXiv:2203.15556},
  year={2022}
}
@article{llama,
  title={LlaMA: Open and efficient foundation language models},
  author={Touvron, Hugo and Lavril, Thibaut and Izacard, Gautier and Martinet, Xavier and Lachaux, Marie-Anne and Lacroix, Timoth{\'e}e and Rozi{\`e}re, Baptiste and Goyal, Naman and Hambro, Eric and Azhar, Faisal and others},
  journal={arXiv preprint arXiv:2302.13971},
  year={2023}
}
@article{lm4rec0,
  title={Personalized prompt learning for explainable recommendation},
  author={Li, Lei and Zhang, Yongfeng and Chen, Li},
  journal={ACM Transactions on Information Systems},
  volume={41},
  number={4},
  pages={1--26},
  year={2023},
  publisher={ACM New York, NY, USA}
}
@inproceedings{lm4rec1,
  title={Recommendation as language processing (rlp): A unified pretrain, personalized prompt \& predict paradigm (p5)},
  author={Geng, Shijie and Liu, Shuchang and Fu, Zuohui and Ge, Yingqiang and Zhang, Yongfeng},
  booktitle={Proceedings of the 16th ACM Conference on Recommender Systems},
  pages={299--315},
  year={2022}
}
@article{lm4rec2,
  title={M6-Rec: Generative Pretrained Language Models are Open-Ended Recommender Systems},
  author={Cui, Zeyu and Ma, Jianxin and Zhou, Chang and Zhou, Jingren and Yang, Hongxia},
  journal={arXiv preprint arXiv:2205.08084},
  year={2022}
}
@article{lm4rec4,
  title={Prompt Learning for News Recommendation},
  author={Zhang, Zizhuo and Wang, Bang},
  journal={arXiv preprint arXiv:2304.05263},
  year={2023}
}
@inproceedings{lm4rec5,
  title={Towards Universal Sequence Representation Learning for Recommender Systems},
  author={Hou, Yupeng and Mu, Shanlei and Zhao, Wayne Xin and Li, Yaliang and Ding, Bolin and Wen, Ji-Rong},
  booktitle={Proceedings of the 28th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={585--593},
  year={2022}
}
@misc{alpaca,
  author = {Rohan Taori and Ishaan Gulrajani and Tianyi Zhang and Yann Dubois and Xuechen Li and Carlos Guestrin and Percy Liang and Tatsunori B. Hashimoto },
  title = {Stanford Alpaca: An Instruction-following LLaMA model},
  year = {2023},
  publisher = {GitHub},
  journal = {GitHub repository},

}
@misc{openaiapi,
   author = {Greg Brockman and Mira Murati and Peter Welinder and OpenAI},
   title = {OpenAI API},

   year = {2022},
}

@inproceedings{prefix,
  author       = {Xiang Lisa Li and
                  Percy Liang},
  title        = {Prefix-Tuning: Optimizing Continuous Prompts for Generation},
  booktitle    = {Proceedings of the 59th Annual Meeting of the Association for Computational
                  Linguistics and the 11th International Joint Conference on Natural
                  Language Processing, {ACL/IJCNLP} 2021, (Volume 1: Long Papers), Virtual
                  Event, August 1-6, 2021},
  pages        = {4582--4597},
  publisher    = {Association for Computational Linguistics},
  year         = {2021},



}

@inproceedings{adapter,
  author       = {Neil Houlsby and
                  Andrei Giurgiu and
                  Stanislaw Jastrzebski and
                  Bruna Morrone and
                  Quentin de Laroussilhe and
                  Andrea Gesmundo and
                  Mona Attariyan and
                  Sylvain Gelly},
  title        = {Parameter-Efficient Transfer Learning for {NLP}},
  booktitle    = {Proceedings of the 36th International Conference on Machine Learning,
                  {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series       = {Proceedings of Machine Learning Research},
  volume       = {97},
  pages        = {2790--2799},
  publisher    = {{PMLR}},
  year         = {2019},


}

@inproceedings{prompt_tuning,
  author       = {Brian Lester and
                  Rami Al{-}Rfou and
                  Noah Constant},

  title        = {The Power of Scale for Parameter-Efficient Prompt Tuning},
  booktitle    = {Proceedings of the 2021 Conference on Empirical Methods in Natural
                  Language Processing, {EMNLP} 2021, Virtual Event / Punta Cana, Dominican
                  Republic, 7-11 November, 2021},
  pages        = {3045--3059},
  publisher    = {Association for Computational Linguistics},
  year         = {2021},



}
@inproceedings{ml-100k,
 author = {F.Maxwell and Joseph A. Konstan},
 year   = {2015},
 title  = { The MovieLens Datasets: History and Context.},
 booktitle = { ACM Transactions on Interactive Intelligent Systems (TiiS)},

}
% F. Maxwell Harper and Joseph A. Konstan. 2015. The MovieLens Datasets: History and Context. ACM Transactions on Interactive Intelligent Systems (TiiS) 5, 4, Article 19 (December 2015), 19 pages. DOI=http://dx.doi.org/10.1145/2827872
